Fairness-enhancing interventions in stream classification

The wide spread usage of automated data-driven decision support systems has raised a lot of concerns regarding accountability and fairness of the employed models in the absence of human supervision. Existing fairness-aware approaches tackle fairness as a batch learning problem and aim at learning a fair model which can then be applied to future instances of the problem. In many applications, however, the data comes sequentially and its characteristics might evolve with time. In such a setting, it is counter-intuitive to "fix" a (fair) model over the data stream as changes in the data might incur changes in the underlying model therefore, affecting its fairness. In this work, we propose fairness-enhancing interventions that modify the input data so that the outcome of any stream classifier applied to that data will be fair. Experiments on real and synthetic data show that our approach achieves good predictive performance and low discrimination scores over the course of the stream.

==> preliminaries.tex <==
%====================================================================================================== 
%\subsection{Discrimination in batch learning}
%We use the original formulation of \cite{kamiran2009classifying}.
%We assume a set of attributes $\{A_1, \cdots, A_n\}$ and their respective domains, $dom(A_i)$, as well as a binary class attribute $Class$.
%We assume a dataset $D$ over a schema $(A_1, \cdots, A_n, C)$, where each instance $x\in D$ is an element of $dom(A_1) \times \cdots \times dom(A_n)$ and class label $c \in dom(C)$.
%Moreover, we assume a special attribute $SA$, referred to as \emph{sensitive attribute} with a special value $s \in dom(SA)$ referred to as \emph{sensitive value} that defines the discriminated community.
%For simplicity, we assume that $SA$ is a binary attribute, i.e., $dom(SA)=\{s,\overline{s}\}$, and we refer to $s$ and $\overline{s}$ as ``deprived'' and ``favored'' communities, respectively. 
%For readability purposes, we also use \{\emph{rejected}, \emph{granted}\} as the class values. 
%We refer to \enquote{granted} class value as \emph{target class}. 
%By combining $SA$ and $C$ (both binary attributes), four communities are created:
%\vspace{-.8cm}
%\begin{table}[ht]\small
	%\centering
		%\caption{Communities based on %\textit{SA} and \textit{Class} %attributes}
	%\label{tab:confusionmatrix}
	%\scalebox{0.8}{
	%\begin{tabular}{ccc}
		%\hline
		%& \multicolumn{2}{c}{\textbf{(true or %predicted) class labels}} \\
		%\begin{tabular}[c]{@{}c@{}}\textbf{Sensi%tive Attribute SA}\end{tabular} & %Rejected & Granted \\ \hline
		%$s$ (Female) & DR \textit{(deprived %rejected)} & DG \textit{(deprived %granted)} \\
		%$\overline{s}$ (Male) & FR %\textit{(favored rejected)} & FG %\textit{(favored granted)} \\ \hline
%	\end{tabular}}
%\end{table}
%\vspace{-0.27cm}

Following the statistical definition of fairness which evaluates whether the probability of being granted is approximately equalized across the different groups~\cite{romei2014multidisciplinary}, also known as \emph{statistical parity}, we formalize discrimination as:
\footnotesize\begin{equation}
\label{eq:static_discReWritten}
disc = \frac{FG}{FG + FR} - \frac{DG}{DG + DR} 
\end{equation}
% \normalsize\noindent
Discrimination can be evaluated for a dataset or for a classifier. In the former case, the real class labels from the dataset $D$ are used in the definition of the different communities (c.f., Table~\ref{tab:confusionmatrix}), whereas in the latter case, the predictions of a classifier $F$ over a dataset $D$ are employed in Table~\ref{tab:confusionmatrix}.
To differentiate the two cases, we use the notation $disc(D)$ and $disc(F,D)$, respectively.

The \emph{discrimination aware classification problem} is to learn a classifier that performs well (i.e., the predictive accuracy is high) and does not discriminate (i.e., the discrimination score, c.f., Equation~\ref{eq:static_discReWritten}, is low). Both predictive accuracy and discrimination scores are evaluated on an independent test set not seen during training.
In general, predictive accuracy and discrimination score are competitive entities and lowering the discrimination might hurt the classification performance~\cite{calders2009building,kamiran2010discrimination,zafar2017fairness}. The goal is to reduce discrimination while hurting classifier's performance as little as possible. 
% The preprocessing approaches for tackling discrimination modify the distribution of the training data so as to allow for a balanced representation of deprived and favored communities in the target class \enquote{granted}. The expectation is that ``correcting'' the data for discrimination will eventually lead into non-discriminating models (though this cannot be guaranteed~\cite{kamiran2012data}).

